Flashy Backdoor: Real-world Environment Backdoor Attack on SNNs with DVS Cameras

While security vulnerabilities in traditional Deep Neural Networks (DNNs) have been extensively studied, the susceptibility of Spiking Neural Networks (SNNs) to adversarial attacks remains mostly underexplored. Until now, the mechanisms to inject backdoors into SNN models have been limited to digital scenarios; thus, we present the first evaluation of backdoor attacks in real-world environments. We begin by assessing the applicability of existing digital backdoor attacks and identifying their limitations for deployment in physical environments. To address each of the found limitations, we present three novel backdoor attack methods on SNNs, i.e., Framed, Strobing, and Flashy Backdoor. We also assess the effectiveness of traditional backdoor procedures and defenses adapted for SNNs, such as pruning, fine-tuning, and fine-pruning. The results show that while these procedures and defenses can mitigate some attacks, they often fail against stronger methods like Flashy Backdoor or sacrifice too much clean accuracy, rendering the models unusable. Overall, all our methods can achieve up to a 100% Attack Success Rate while maintaining high clean accuracy in every tested dataset. Additionally, we evaluate the stealthiness of the triggers with commonly used metrics, finding them highly stealthy. Thus, we propose new alternatives more suited for identifying poisoned samples in these scenarios. Our results show that further research is needed to ensure the security of SNN-based systems against backdoor attacks and their safe application in real-world scenarios. The code, experiments, and results are available in our repository.

==> sections/old_evaluation.tex <==

\subsection{Experimental Results}

We evaluate the attacks with commonly used metrics:
\begin{compactenum}
    \item ASR measures the backdoor performance of the model based on a holdout fully backdoored dataset. We also ensure that for all the poisoned samples $\hat{\textbf{x}}$ the original label $y$ was different from the objective label $\hat{y}$ if there were any $\hat{\textbf{x}}\in {D}_{ps}$ where $y = \hat{y}$, we would substitute the sample with another one to ensure the correct measurement of the ASR.\todo{unclear}
    \item Clean accuracy measures the model's performance on a holdout clean dataset.
\end{compactenum}


\begin{table}[ht]
\centering
\caption{Comparison of the results with different trigger sizes of polarity $p=1$ inserted at the start in the DVS128-Gesture dataset.}\label{tab:1}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{ASR\%} & \textbf{Clean ACC\%} & \textbf{Trigger length} & \textbf{Trigger size\%} \\ \midrule
12.38 $\pm$ 0.05 & 90.16 $\pm$ 0.02 & 5 & 10 \\
63.43 $\pm$ 41.36 & 89.0 $\pm$ 0.08 & 6 & 10 \\
15.51 $\pm$ 0.22 & 90.51 $\pm$ 0.05 & 7 & 10 \\
58.68 $\pm$ 26.12 & 90.28 $\pm$ 0.03 & 8 & 10 \\ \midrule
13.54 $\pm$ 0.19 & 89.58 $\pm$ 0.04 & 3 & 20 \\
60.53 $\pm$ 37.85 & 89.12 $\pm$ 0.15 & 4 & 20 \\
71.88 $\pm$ 44.58 & 88.89 $\pm$ 0.07 & 5 & 20 \\
75.46 $\pm$ 36.12 & 90.74 $\pm$ 0.06 & 6 & 20 \\ \midrule
13.54 $\pm$ 0.09 & 88.43 $\pm$ 0.06 & 2 & 30 \\
40.97 $\pm$ 51.67 & 89.35 $\pm$ 0.13 & 3 & 30 \\
88.77 $\pm$ 7.56 & 90.39 $\pm$ 0.01 & 4 & 30 \\
100 $\pm$ 0.0 & 91.2 $\pm$ 0.02 & 7 & 30 \\ \midrule
19.33 $\pm$ 0.53 & 88.89 $\pm$ 0.05 & 1 & 100 \\
98.84 $\pm$ 0.04 & 90.62 $\pm$ 0.0 & 2 & 100 \\
100 $\pm$ 0.0 & 90.62 $\pm$ 0.03 & 3 & 100 \\
100 $\pm$0.0 & 92.82 $\pm$0.03 & 4 & 100 \\ \bottomrule
\end{tabular}

\end{table}

All attacks were tested on each dataset three times, and the standard deviation (STD) was measured to account for variability. Please note that all additional graphs and experimental results have been relocated to~\autoref{appendixA} to facilitate ease of reading.

\begin{table}[ht]
\centering
\caption{Comparison of the results with different temporal locations of the trigger with polarity $p=1$ and size of 100\% of the original frame on DVS128-Gesture dataset}\label{tab:2}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{ASR\%} & \textbf{Clean ACC \%} & \multicolumn{1}{c}{\textbf{Trigger length}} & \textbf{Position} \\ \midrule
19.33 $\pm$ 0.53 & 88.89 $\pm$ 0.05 & 1 & Start \\
98.84 $\pm$ 0.04 & 90.62 $\pm$ 0.0 & 2 & Start \\
100 $\pm$ 0.0 & 90.62 $\pm$ 0.03 & 3 & Start \\ \midrule
47.34 $\pm$ 19.35 & 90.05 $\pm$ 0.01 & 1 & Middle \\
99.54 $\pm$ 0.01 & 91.67 $\pm$ 0.0 & 2 & Middle \\
100 $\pm$ 0.0 & 92.59 $\pm$ 0.0 & 3 & Middle \\ \midrule
11.11 $\pm$ 0.01 & 88.77 $\pm$ 0.01 & 1 & End \\
24.65 $\pm$ 0.25 & 90.74 $\pm$ 0.01 & 6 & End \\
86.0 $\pm$ 6.15 & 91.55 $\pm$ 0.05 & 8 & End \\ \bottomrule
\end{tabular}
\end{table}

\subsection{Framed Backdoor}

To assess the viability of the proposed attack, we first experiment with the BadNets~\cite{BadNets} approach, but limiting the position of the trigger to the upper-left corner and maintaining a constant poisoning rate $\epsilon$ of $0.1$. Then, we introduced the trigger in different time sections of the samples (start, middle, or end), with trigger duration ranging from 1 to 8 frames and four different trigger sizes: 10\%, 20\%, 30\%, and 100\% of the original image. The previously mentioned limitations allowed us to carefully examine the effect these parameters have on the resulting ASR as well as the clean accuracy of the model.

Our experiments reveal that the trigger's size is inversely correlated with the number of frames required to perform the backdoor effectively. When the trigger is the largest and presented at the start or middle, the attack achieved a 100\% ASR in all tested datasets for every possible polarity. Furthermore, in the most efficient polarities, it can be observed that the system is capable of achieving 100\% ASR accuracy within a mere 2 to 3 frames (see~\autoref{fig:gestures_graphs}). Increasing the trigger's size also increased the stability of the results (see~\autoref{tab:1}). Notably, every attack we tested maintained the same clean accuracy for all cases studied (see~\autoref{fig:gestures_graphs}). We also observe that the temporal position affects the attack's effectiveness, performing worse the later it is introduced (see~\autoref{tab:2}). However, further testing is required to determine the cause of this.\todo{some hypothesis?}

\begin{table}[ht]
\centering
\caption{Comparison of the results with different trigger sizes of polarity $p=1$ inserted at the start in the DVS128-Gesture dataset with a gap of 1 clean frame between each 2 poisoned frames.}\label{tab:3}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{ASR\%} & \textbf{Clean ACC \%} & \multicolumn{1}{c}{\textbf{P frames}} & \multicolumn{1}{c}{\textbf{Trigger Size \%}} \\ \midrule
10.76 $\pm$ 0.02 & 89.35 $\pm$ 0.06 & 3 & 10 \\
11.11 $\pm$ 0.01 & 88.54 $\pm$ 0.07 & 4 & 10 \\
11.23 $\pm$ 0.02 & 88.77 $\pm$ 0.07 & 5 & 10 \\
12.15 $\pm$ 0.07 & 88.19 $\pm$ 0.07 & 6 & 10 \\ \midrule
12.15 $\pm$ 0.14 & 89.12 $\pm$ 0.1 & 3 & 20 \\
50.69 $\pm$ 40.72 & 90.16 $\pm$ 0.11 & 4 & 20 \\
51.27 $\pm$ 39.77 & 89.12 $\pm$ 0.07 & 5 & 20 \\
70.37 $\pm$ 52.67 & 90.86 $\pm$ 0.03 & 6 & 20 \\ \midrule
12.85 $\pm$ 0.07 & 89.00 $\pm$ 0.18 & 2 & 30 \\
71.53 $\pm$ 48.64 & 91.32 $\pm$ 0.09 & 5 & 30 \\
99.88 $\pm$ 0.0 & 91.44 $\pm$ 0.01 & 6 & 30 \\ \midrule
19.33 $\pm$ 0.53 & 88.89 $\pm$ 0.05 & 1 & 100 \\
100 $\pm$ 0.0 & 91.67 $\pm$ 0.06 & 2 & 100 \\
100 $\pm$ 0.0 & 91.44 $\pm$ 0.03 & 3 & 100 \\
100 $\pm$ 0.0 & 92.25 $\pm$ 0.02 & 4 & 100 \\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\caption{Comparison of the results with different temporal locations of the trigger with polarity $p=1$ and a size of 100\% of the original frame on the DVS128-Gesture dataset with a gap of 1 clean frame between each 2 poisoned frames.}\label{tab:4}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{ASR\%} & \textbf{Clean ACC \%} & \textbf{P frames} & \textbf{Position} \\ \midrule
19.33 $\pm$ 0.53 & 88.89 $\pm$ 0.05 & 1 & Start \\
100 $\pm$ 0.0 & 91.67 $\pm$ 0.06 & 2 & Start \\
100 $\pm$ 0.0 & 91.44 $\pm$ 0.03 & 3 & Start \\ \midrule
47.34 $\pm$ 19.35 & 90.05 $\pm$ 0.01 & 1 & Middle \\
99.88 $\pm$ 0.0 & 91.90 $\pm$ 0.01 & 2 & Middle \\
100 $\pm$ 0.0 & 92.13 $\pm$ 0.02 & 3 & Middle \\ \midrule
11.11 $\pm$ 0.01 & 88.77 $\pm$ 0.01 & 1 & End \\
50.93 $\pm$ 0.34 & 90.62 $\pm$ 0.01 & 4 & End \\
100 $\pm$ 0.0 & 91.20 $\pm$ 0.02 & 5 & End \\ \bottomrule
\end{tabular}
\end{table}

\subsection{Strobing Backdoor}

The next step is to analyze the effect a non-continuous trigger has on the model performance. We maintain the same limitations as in the previous test, but this time, we introduce a clean frame between each pair of poisoned frames. We proceed again to introduce the trigger in each time section with trigger duration ranging from 3 to 13 frames; note that half of the trigger frames are clean frames, so there could only be $\lceil trigger\_length/2 \rceil$ poisoned frames in any sample.

Our testing shows that the attack's performance is mostly equal or occasionally better when the trigger is positioned at the start or middle (see~\autoref{tab:3} and~\autoref{fig:gestures_graphs_strobe}), without observing any degradation in the clean accuracy (see~\autoref{tab:3} and~\autoref{fig:gestures_graphs_strobe}). However, when positioned at the end, its performance increases compared to the \emph{Framed Backdoor} (see~\autoref{tab:4}).
This approach also enhances the attack's stealthiness, as it requires the trigger to be present in fewer frames than its continuous counterpart, and it yields improved performance in cases where the trigger is not present at the start (see~\autoref{tab:3} and~\autoref{fig:gestures_graphs_strobe}).

After doing a hyperparameter analysis, we conclude that modifying the trigger gap does not have any substantial effect on the clean accuracy. However, it positively affects ASR when the trigger is positioned at the end. Still, careful consideration of the gap is needed, as it can also make the training less stable for the backdoor behavior, and significant gaps can have the opposite effect on ASR (see~\autoref{tab:gap_analisis}).


\begin{table}[ht]
\centering
\caption{Results of the hyperparameter analysis of the gap length in the DVS128-Gesture dataset, with a gap size ranging from 1 to 4 and the trigger introduced at the Start, Middle, or End of the poisoned samples with 3 poisoned frames with triggers of size 20\% on each one.}
\label{tab:gap_analisis}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{ASR\%} & \textbf{Clean ACC \%} & \textbf{Gap size} & \textbf{Position} \\ \midrule
98.95 $\pm$ 0.35 & 90.27 $\pm$ 0.006 & 1 & START \\
96.41 $\pm$ 2.56 & 91.66 $\pm$ 0.015 & 2 & START \\
69.44 $\pm$ 48.45 & 90.27 $\pm$ 0.015 & 3 & START \\
94.90 $\pm$ 5.85 & 91.12 $\pm$ 0.005 & 4 & START \\ \midrule
99.07 $\pm$ 0.20 & 92.36 $\pm$ 0.017 & 1 & MID \\
99.07 $\pm$ 0.20 & 91.08 $\pm$ 0.011 & 2 & MID \\
99.18 $\pm$ 0.20 & 90.74 $\pm$ 0.012 & 3 & MID \\
40.27 $\pm$ 41.80 & 89.35 $\pm$ 0.026 & 4 & MID \\ \midrule
18.17 $\pm$ 5.08 & 89.00 $\pm$ 0.017 & 1 & END \\
18.28 $\pm$ 7.02 & 89.12 $\pm$ 0.019 & 2 & END \\
75.34 $\pm$ 34.71 & 90.85 $\pm$ 0.008 & 3 & END \\
80.32 $\pm$ 31.39 & 90.16 $\pm$ 0.017 & 4 & END \\ \bottomrule
\end{tabular}
\end{table}


\subsection{Flashy Backdoor}

We merge both concepts presented in the previous attacks, the framing and the strobing, but this time, we fix the trigger size to 100\% of the original frames and ensure there is at least a clean frame between two poisoned frames. This approach ensures that the DVS camera has time to reset its threshold (see~\autoref{fig:PoisonframeDVS}) while making the triggers reproducible in real-world scenarios.

As shown in~\autoref{tab:1} and~\autoref{tab:3}, our results suggest that combining the full-frame size trigger with the benefits of strobing results in better ASR in every scenario while maintaining the same or even achieving superior clean accuracy in all cases. These results suggest that it is better to concentrate the trigger in fewer frames rather than spreading it through the sample. As can be seen in~\autoref{tab:1}, poisoning 30\% of the first 4 frames of the samples obtains substantially better results than poisoning 20\% of 6 frames, even if the poisoning relative to the total amount of pixels in the samples is the same. Additionally, \autoref{tab:2} and~\autoref{tab:4} show that separating the frames in which the trigger is inserted can make the insertion of the backdoor more stable and perform better when inserted in later temporal locations, making it easier to deploy in physical scenarios. Thus, we conclude that apart from being a necessary step for the transference to real-world environments, introducing a full-frame strobing flash is also beneficial in digital scenarios for both the performance and the stability of the attack.

Lastly, we transfer this attack to a physical environment. As our DVS camera had different specifications compared to the one used to capture the DVS128-Gesture dataset, we first started by ensuring our model was able to identify our newly captured samples correctly. Similarly to the original dataset, each sample we captured lasts around 6 seconds. After cropping the samples to a size of 512 $\times$ 512 pixels, we downscaled them to 128 $\times$ 128 pixels to feed them into the network trained in the original dataset. We capture both clean and poisoned samples with our DVS camera; the captured samples consist of 4 different subjects, with a total of 89 clean samples and 78 poisoned samples.

Then, we test the initial accuracy of a clean network to validate subsequent\todo{which are those?} results (see~\autoref{tab:real-world}), obtaining an accuracy of 76.40\% in our clean samples with an ASR of 8.97\% and an accuracy of 61.53\% in the poisoned samples. Note this is normal as the model can mistakenly guess the trigger label by chance when predicting any other sample, but with its initial clean accuracy this result is not significant enough to determine that the model tends to predict our trigger label more than any other.\todo{unclear, I split original sentence into two and it is still too long} 

\todo{what is base ASR?}

\begin{table}
\centering
\caption{Results on real-world samples of the digitally trained models, including a baseline of a clean model measuring the clean accuracy on both clean and poisoned samples (marked with *) and the base ASR.}
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Polarity} & \textbf{Trigger\_length} & \multicolumn{2}{c}{\textbf{Clean acc\%}} & \textbf{ASR\%} \\ \midrule
Baseline          & Baseline                 & 76.40    & 61.53* & 8.97           \\ \midrule
1                 & 1                        & \multicolumn{2}{c}{73.03 $\pm$ 3.37}         & 38.45 $\pm$ 23.11  \\
2                 & 1                        & \multicolumn{2}{c}{53.17 $\pm$ 13.96}        & 65.38 $\pm$ 8.97   \\
3                 & 1                        & \multicolumn{2}{c}{67.79 $\pm$ 3.37}         & 31.96 $\pm$ 30.07  \\ \midrule
1                 & 3                        & \multicolumn{2}{c}{72.65 $\pm$ 3.43}         & 45.72 $\pm$ 34.88  \\
2                 & 3                        & \multicolumn{2}{c}{60.29 $\pm$ 2.34}         & 60.68 $\pm$ 4.50   \\
3                 & 3                        & \multicolumn{2}{c}{71.53 $\pm$ 2.59}         & 97.86 $\pm$ 3.70   \\ \midrule
1                 & 5                        & \multicolumn{2}{c}{70.03 $\pm$ 2.34}         & 43.58 $\pm$ 35.89  \\
2                 & 5                        & \multicolumn{2}{c}{50.18 $\pm$ 11.69}        & 66.23 $\pm$ 8.33   \\
3                 & 5                        & \multicolumn{2}{c}{70.03 $\pm$ 0.64}         & 90.16 $\pm$ 4.85   \\ \bottomrule
\end{tabular}
\label{tab:real-world}
\end{table}

After ensuring that our clean model can correctly identify our real-world samples, we train different models based on the results obtained in the digital scenarios, with polarities $p\in[1,2,3]$. Our resulting models are trained with poisoned samples of trigger length between $3$ and $5$ inserted at the start and a gap of size of $1$ between each poisoned frame (essentially containing between 1 and 3 poisoned frames).\todo{?}

We test each of the models and observe that the best results are obtained when the trigger polarity is set at $p=3$, meaning that the triggers contained both ON and OFF events, achieving nearly 100\% ASR with little variance when the digital trigger length adapts best to out real triggers (see~\autoref{tab:real-world}). This was to be expected, as most of the poisoned samples captured in the real world contained both in the trigger frames. Nevertheless, we were able to introduce the backdoor behavior with all polarities, even when the trigger did not perfectly match the digital one. This could be seen as a bad thing because it could be accidentally triggered when the attacker does not intend to, but in a real-world scenario, it makes it easier to attack the model reliably.\todo{unclear} 

After analyzing the results, we also noticed that increasing the trigger length can result in higher ASR. However, it is necessary to carefully determine the best length, as slightly increasing it can positively affect clean accuracy, but increasing it too much can also result in a degradation of the clean accuracy depending on the settings. We also notice that, in general, polarity $p=1$ yields the best results in clean accuracy but the worst in ASR. This is due to the triggers having a mix of ON and OFF activations in the majority of the frames, and thus, the model is not able to correctly discern the trigger.
Nevertheless, it is possible to effectively introduce the backdoor behavior while mostly maintaining the initial clean accuracy regardless of the settings, achieving very high clean accuracy and ASR when carefully mimicking the triggers. Thus, we conclude that it is feasible to train a backdoored model with digital triggers and attack the model in real-world scenarios without the need to introduce any real\todo{?} trigger sample in the training data or perfectly match the digital trigger. 

\subsection{Evaluation against Backdoor Defenses}

Given the lack of specific backdoor defenses for SNNs, we experiment with two commonly used methods in DL that have been studied as a means to enhance the security of already trained models, i.e., pruning and fine-tuning, and implement a defense from the DNN domain to work with neuromorphic data in SNNs: fine-pruning~\cite{fine_prune}. To test the effectiveness of both methods and the defense in real-world environments, we select the best-performing model based on ASR, clean accuracy, and the results obtained from the defenses applied to the models with digital samples. The selected model is the best one trained with polarity $p=3$, trigger length 3, and a clean gap of 1, as this represents the worst-case scenario between the tested ones.

\subsubsection{Pruning}

Pruning has been commonly used to reduce the computational expense of DNNs~\cite{pruning_1, pruning_2, pruning_3}, showing that a significant amount of neurons can be pruned before starting to compromise the classification accuracy. However, it was also explored as a method to enhance the security of corrupt DNNs by Liu et al.~\cite{fine_prune}.
The premise behind this defense is that the attacked model learns to misbehave on backdoored inputs while behaving correctly on clean inputs because there are ``backdoor neurons'' that remain dormant in the presence of clean inputs but activate under the presence of the specified trigger, which was empirically demonstrated by Gu et al.~\cite{backdoor_neurons}.

The pruning defense operates as follows. First, an evaluation of the network under clean inputs from the test dataset is performed. Then, the mean activation of the final convolutional layer is computed, focusing on this final layer due to its proximity to the output layer, as it contains features more specific to the task, including the backdoor behavior. The next step is to rank the neurons based on their mean activations from lower to higher and prune a percentage of those neurons based on the pruning rate $\tau$. This methodology is employed because Liu et al.~\cite{fine_prune} found that in practice, the neurons with the lowest mean activations are not triggered by either clean or backdoored data, having no impact on either the clean accuracy or the ASR of the model. Those are followed mainly by neurons that activate under backdoored data but not clean inputs; pruning them results in a reduction of ASR without compromising the clean accuracy. The last neurons are the ones that activate only under benign samples.

\begin{table*}[b]
\centering
\caption{Results of the pruning procedure with a pruning rate of 0.8 for all the presented attacks and the DVS128-Gesture, NMnist, and Cifar10-DVS datasets.
}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Size} & \textbf{Attack} & \textbf{P Frames} & \textbf{Ini CA\%} & \textbf{I ASR\%} & \textbf{$\tau$} & \textbf{Pruned CA\%} & \textbf{Pruned ASR\%} \\ \midrule
DVS128-Gesture & 0.3 & Static & 16 & 90.62 $\pm$ 0.35 & 99.08 $\pm$ 0.40        & 0.8 & 24.31 $\pm$ 13.02 & 9.38 $\pm$ 13.84 \\
DVS128-Gesture & 0.3 & Framed & 12 & 91.20 $\pm$ 1.00 & 99.08 $\pm$ 0.20        & 0.8 & 31.60 $\pm$ 3.67 & 8.94 $\pm$ 11.09 \\
DVS128-Gesture & 0.3 & Framed & 6 & 89.47 $\pm$ 1.56 & 54.63 $\pm$ 35.50        & 0.8 & 41.90 $\pm$ 5.88 & 9.49 $\pm$ 14.94 \\
DVS128-Gesture & 0.3 & Strobing & 6 & 89.00 $\pm$ 1.56 & 97.80 $\pm$ 0.87       & 0.8 & 22.55 $\pm$ 3.75 & 0.70 $\pm$ 0.92 \\
DVS128-Gesture & 1 & Flash & 6 & 90.20 $\pm$ 0.92 & 99.54 $\pm$ 0.53            & 0.8 & 48.38 $\pm$ 12.14 & 99.54 $\pm$ 0.80 \\
DVS128-Gesture & 1 & Flash & 3 & 87.61 $\pm$ 1.91 & 96.64 $\pm$ 4.07            & 0.8 & 36.81 $\pm$ 15.14 & 69.91 $\pm$ 40.36 \\
DVS128-Gesture & 1 & Strobing Flash & 3 & 88.31 $\pm$ 2.81 & 90.28 $\pm$ 15.04  & 0.8 & 35.53 $\pm$ 7.46 & 55.90 $\pm$ 42.02 \\ \midrule
NMnist & 0.3 & Static & 16 & 99.28 $\pm$ 0.03 & 99.97 $\pm$ 0.00                & 0.8 & 88.60 $\pm$ 9.19 & 99.35 $\pm$ 0.97 \\
NMnist & 0.3 & Framed & 10 & 99.28 $\pm$ 0.03 & 99.97 $\pm$ 0.00                & 0.8 & 85.20 $\pm$ 7.74 & 99.06 $\pm$ 0.60 \\
NMnist & 0.3 & Framed & 5 & 99.24 $\pm$ 0.03 & 99.97 $\pm$ 0.01                 & 0.8 & 92.28 $\pm$ 2.80 & 81.37 $\pm$ 28.70 \\
NMnist & 0.3 & Strobing & 5 & 99.29 $\pm$ 0.04 & 99.97 $\pm$ 0.01               & 0.8 & 79.21 $\pm$ 6.95 & 98.33 $\pm$ 2.67 \\
NMnist & 1 & Flash & 6 & 99.29 $\pm$ 0.03 & 99.97 $\pm$ 0.02                    & 0.8 & 89.01 $\pm$ 4.40 & 69.82 $\pm$ 52.05 \\
NMnist & 1 & Flash & 3 & 99.27 $\pm$ 0.02 & 99.97 $\pm$ 0.00                    & 0.8 & 94.40 $\pm$ 2.09 & 78.06 $\pm$ 25.44 \\
NMnist & 1 & Strobing Flash & 3 & 99.30 $\pm$ 0.02 & 99.96 $\pm$ 0.01           & 0.8 & 87.26 $\pm$ 9.32 & 69.35 $\pm$ 48.22 \\ \midrule
Cifar10-DVS & 0.3 & Static & 16 & 67.47 $\pm$ 0.78 & 95.83 $\pm$ 0.06           & 0.8 & 33.27 $\pm$ 1.63 & 70.80 $\pm$ 16.75 \\
Cifar10-DVS & 0.3 & Framed & 10 & 67.30 $\pm$ 0.90 & 95.67 $\pm$ 0.06           & 0.8 & 27.53 $\pm$ 0.74 & 92.67 $\pm$ 2.25 \\
Cifar10-DVS & 0.3 & Framed & 5 & 66.33 $\pm$ 0.61 & 95.60 $\pm$ 0.10            & 0.8 & 28.07 $\pm$ 2.11 & 94.40 $\pm$ 0.92 \\
Cifar10-DVS & 0.3 & Strobing & 5 & 66.20 $\pm$ 0.72 & 95.57 $\pm$ 0.21          & 0.8 & 30.23 $\pm$ 2.25 & 94.80 $\pm$ 2.30 \\
Cifar10-DVS & 1 & Flash & 6 & 63.40 $\pm$ 0.98 & 95.87 $\pm$ 0.15               & 0.8 & 11.07 $\pm$ 1.22 & 99.90 $\pm$ 0.17 \\
Cifar10-DVS & 1 & Flash & 3 & 63.97 $\pm$ 0.93 & 95.57 $\pm$ 0.42               & 0.8 & 17.20 $\pm$ 9.68 & 98.50 $\pm$ 2.18 \\
Cifar10-DVS & 1 & Strobing Flash & 3 & 64.47 $\pm$ 1.12 & 95.53 $\pm$ 0.21      & 0.8 & 12.30 $\pm$ 3.64 & 99.87 $\pm$ 0.23 \\\bottomrule
\end{tabular}
}
\end{table*}
\todo{R: I could merge tables 7,8 and 9 as the 6 first columns are the same for all, but it would get a bit cramped I think. See examples \autoref{table11}, \autoref{table12}, \autoref{table13}}
% \begin{table*}[b]
% \centering
% \caption{Results of the pruning defense with a prune rate of 0.8 for all the presented attacks in the DVS128-Gesture, NMnist, and Cifar10-DVS datasets.}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \textbf{Dataset} & \textbf{Size} & \textbf{Attack} & \textbf{P Frames} & \textbf{Ini CA\%} & \textbf{I ASR\%} & \textbf{$\tau$} & \textbf{Pruned CA\%} & \textbf{Pruned ASR\%} \\ \midrule
% DVS128-Gesture & 0.3 & Static & 16 & 92.71& 99.31& 0.8 & 26.97 $\pm$ 0.20 & 99.88 $\pm$ 0.0 \\
% DVS128-Gesture & 0.3 & Framed & 12 & 92.36& 99.31& 0.8 & 21.06 $\pm$ 0.19 & 95.25 $\pm$ 0.08 \\
% DVS128-Gesture & 0.3 & Framed & 6 & 91.67& 99.42& 0.8 & 9.38 $\pm$ 0.02 & 100 $\pm$ 0.0 \\
% DVS128-Gesture & 0.3 & Strobing & 6 & 92.01& 99.31& 0.8 & 36.00 $\pm$ 0.09 & 93.29 $\pm$ 0.02 \\
% DVS128-Gesture & 1 & Flash & 6 & 92.71& 99.42& 0.8 & 11.11 $\pm$ 0.05 & 100 $\pm$ 0.0 \\
% DVS128-Gesture & 1 & Flash & 3 & 91.90& 98.96& 0.8 & 26.27 $\pm$ 0.11 & 100 $\pm$ 0.0 \\
% DVS128-Gesture & 1 & Strobing Flash & 3 & 88.19& 99.65& 0.8 & 17.36 $\pm$ 0.10 & 100 $\pm$ 0.0 \\ \midrule
% NMnist & 0.3 & Static & 16 & 99.49& 99.98& 0.8 & 95.24 $\pm$ 0.03 & 99.76 $\pm$ 0.0 \\
% NMnist & 0.3 & Framed & 10 & 99.46& 99.98& 0.8 & 96.26 $\pm$ 0.02 & 96.65 $\pm$ 0.06 \\
% NMnist & 0.3 & Framed & 5 & 99.42& 99.97& 0.8 & 96.32 $\pm$ 0.02 & 92.51 $\pm$ 0.10 \\
% NMnist & 0.3 & Strobing & 5 & 99.46& 99.98& 0.8 & 95.87 $\pm$ 0.03 & 72.90 $\pm$ 0.47 \\
% NMnist & 1 & Flash & 6 & 99.47& 99.97& 0.8 & 95.10 $\pm$ 0.02 & 68.18 $\pm$ 0.52 \\
% NMnist & 1 & Flash & 3 & 99.44& 99.98& 0.8 & 95.21 $\pm$ 0.02 & 99.55 $\pm$ 0.0 \\
% NMnist & 1 & Strobing Flash & 3 & 99.44& 99.98& 0.8 & 94.79 $\pm$ 0.03 & 38.79 $\pm$ 0.42 \\ \midrule
% Cifar10-DVS & 0.3 & Static & 16 & 67.57& 95.57& 0.8 & 13.57 $\pm$ 0.04 & 28.07 $\pm$ 0.48 \\
% Cifar10-DVS & 0.3 & Framed & 10 & 67.87& 95.67& 0.8 & 14.07 $\pm$ 0.06 & 52.00 $\pm$ 0.42 \\
% Cifar10-DVS & 0.3 & Framed & 5 & 67.10& 95.43& 0.8 & 16.83 $\pm$ 0.07 & 10.10 $\pm$ 0.17 \\
% Cifar10-DVS & 0.3 & Strobing & 5 & 67.17& 95.80& 0.8 & 15.80 $\pm$ 0.05 & 35.80 $\pm$ 0.52 \\
% Cifar10-DVS & 1 & Flash & 6 & 65.10& 96.27& 0.8 & 11.60 $\pm$ 0.03 & 99.97 $\pm$ 0.0 \\
% Cifar10-DVS & 1 & Flash & 3 & 63.07& 96.37& 0.8 & 15.57 $\pm$ 0.09 & 98.43 $\pm$ 0.03 \\
% Cifar10-DVS & 1 & Strobing Flash & 3 & 65.70& 96.23& 0.8 & 16.37 $\pm$ 0.01 & 43.47 $\pm$ 0.50 \\ \midrule
% Real-samples & 1 & Strobing flash & 2 & 73.03& 100& 0.8 &  8.98 $\pm$ 0.0  &  100 $\pm$ 0.0  \\\bottomrule
% \end{tabular}
% }
% \label{tab:prune_defense}
% \end{table*}

% \begin{table*}[b]
% \centering
% \caption{Results of the pruning defense with a prune rate of 0.8 for all the presented attacks in the DVS128-Gesture, NMnist, and Cifar10-DVS datasets.}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \textbf{Dataset} & \textbf{Size} & \textbf{Attack} & \textbf{P Frames} & \textbf{Ini CA\%} & \textbf{I ASR\%} & \textbf{$\tau$} & \textbf{Pruned CA\%} & \textbf{Pruned ASR\%} \\ \midrule
% DVS128-Gesture & 0.3 & Static & 16 & 92.71 & 99.31 & 0.8 & 26.97 $\pm$ 0.20 & 99.88 $\pm$ 0.0 \\
% DVS128-Gesture & 0.3 & Framed & 12 & 92.36 & 99.31 & 0.8 & 21.06 $\pm$ 0.19 & 95.25 $\pm$ 0.08 \\
% DVS128-Gesture & 0.3 & Framed & 6 & 91.67 & 99.42 & 0.8 & 9.38 $\pm$ 0.02 & 100 $\pm$ 0.0 \\
% DVS128-Gesture & 0.3 & Strobing & 6 & 92.01 & 99.31 & 0.8 & 36.00 $\pm$ 0.09 & 93.29 $\pm$ 0.02 \\
% DVS128-Gesture & 1 & Flash & 6 & 92.71 & 99.42 & 0.8 & 11.11 $\pm$ 0.05 & 100 $\pm$ 0.0 \\
% DVS128-Gesture & 1 & Flash & 3 & 91.90 & 98.96 & 0.8 & 26.27 $\pm$ 0.11 & 100 $\pm$ 0.0 \\
% DVS128-Gesture & 1 & Strobing Flash & 3 & 88.19 & 99.65 & 0.8 & 17.36 $\pm$ 0.10 & 100 $\pm$ 0.0 \\ \midrule
% NMnist & 0.3 & Static & 16 & 99.49 & 99.98 & 0.8 & 95.24 $\pm$ 0.03 & 99.76 $\pm$ 0.0 \\
% NMnist & 0.3 & Framed & 10 & 99.46 & 99.98 & 0.8 & 96.26 $\pm$ 0.02 & 96.65 $\pm$ 0.06 \\
% NMnist & 0.3 & Framed & 5 & 99.42 & 99.97 & 0.8 & 96.32 $\pm$ 0.02 & 92.51 $\pm$ 0.10 \\
% NMnist & 0.3 & Strobing & 5 & 99.46 & 99.98 & 0.8 & 95.87 $\pm$ 0.03 & 72.90 $\pm$ 0.47 \\
% NMnist & 1 & Flash & 6 & 99.47 & 99.97 & 0.8 & 95.10 $\pm$ 0.02 & 68.18 $\pm$ 0.52 \\
% NMnist & 1 & Flash & 3 & 99.44 & 99.98 & 0.8 & 95.21 $\pm$ 0.02 & 99.55 $\pm$ 0.0 \\
% NMnist & 1 & Strobing Flash & 3 & 99.44 & 99.98 & 0.8 & 94.79 $\pm$ 0.03 & 38.79 $\pm$ 0.42 \\ \midrule
% Cifar10-DVS & 0.3 & Static & 16 & 67.57 & 95.57 & 0.8 & 13.57 $\pm$ 0.04 & 28.07 $\pm$ 0.48 \\
% Cifar10-DVS & 0.3 & Framed & 10 & 67.87 & 95.67 & 0.8 & 14.07 $\pm$ 0.06 & 52.00 $\pm$ 0.42 \\
% Cifar10-DVS & 0.3 & Framed & 5 & 67.10 & 95.43 & 0.8 & 16.83 $\pm$ 0.07 & 10.10 $\pm$ 0.17 \\
% Cifar10-DVS & 0.3 & Strobing & 5 & 67.17 & 95.80 & 0.8 & 15.80 $\pm$ 0.05 & 35.80 $\pm$ 0.52 \\
% Cifar10-DVS & 1 & Flash & 6 & 65.10 & 96.27 & 0.8 & 11.60 $\pm$ 0.03 & 99.97 $\pm$ 0.0 \\
% Cifar10-DVS & 1 & Flash & 3 & 63.07 & 96.37 & 0.8 & 15.57 $\pm$ 0.09 & 98.43 $\pm$ 0.03 \\
% Cifar10-DVS & 1 & Strobing Flash & 3 & 65.70 & 96.23 & 0.8 & 16.37 $\pm$ 0.01 & 43.47 $\pm$ 0.50 \\ \midrule
% Real-samples & 1 & Strobing flash & 2 & 73.03 & 100 & 0.8 &  8.98 $\pm$ 0.0  &  100 $\pm$ 0.0  \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:prune_defense}
% \end{table*}

We apply this procedure with a pruning rate of $\tau = 0.8$, meaning that 80\% of the neurons in the model are pruned, and focus on the effect that the length of the trigger (from 3 to 16 poisoned frames) and the clean gap between each trigger has in each proposed attack on the DVS128-Gesture, NMnist, and Cifar10-DVS datasets (see~\autoref{tab:prune_defense}). As can be seen, even though the initial clean accuracy and ASR are high before pruning, we observe a substantial decrease in the clean accuracy across all datasets (except on NMnist, where the drop is less noticeable) after pruning.

In general, we observe that the defense has little effect when pruning this amount of neurons on all datasets, except DVS128-Gesture when the trigger sizes are small. It can also be seen that the increase in the trigger size and number of poisoned frames is positively related to the resistance of the ASR.

The pruning defense effectively reduces ASR for attacks with smaller trigger sizes on the DVS128-Gesture dataset.\todo{this is already said two sentences before} 
However, this reduction in ASR also comes linked to a substantial decrease in clean accuracy, losing more than 75\% in some cases. For attacks with larger trigger sizes, the procedure is less effective, losing most of the clean accuracy while not being able to eliminate the backdoor behavior. This suggests that the larger the trigger, the deeper it is embedded in the model, making pruning less capable of removing it without compromising the model's performance.

For the NMnist dataset, pruning demonstrates limited effectiveness in reducing ASR, which remains high after pruning, often above 78\%, regardless of the trigger size. Although the clean accuracy decreases following pruning, it stays relatively high compared to other datasets, remaining above 79\% in most cases. This suggests that the model contains many redundant neurons that do not significantly impact the results; therefore, pruning them does not produce a substantial effect.
For the Cifar10-DVS dataset, the pruning defense appears ineffective in reducing ASR across all attacks, especially those with larger trigger sizes. The ASR remains high after pruning, often above 90\%, regardless of the trigger length or attack type, while the clean accuracy drops significantly, from around 66\% to as low as 11\%.

After analyzing these results, a general tendency can be observed, as pruned models trained with bigger triggers tend to have a more substantial drop in clean accuracy and less impact on ASR. This outcome was expected; a smaller trigger can be more discrete, but it also has less impact on the model, mainly injecting the backdoor on less influential neurons. The pruning process first focuses on removing these less influential neurons, making it easier to erase the backdoor behavior. However, with the introduction of larger triggers, their influence on the model is also amplified, making them more challenging to target through pruning.

% We apply this procedure with a pruning rate of $\tau = 0.8$, meaning that 80\% of the neurons in the model are pruned, and focus on the effect that the length of the trigger (from 3 to 16 poisoned frames) and the clean gap between each trigger has in each proposed attack on the DVS128-Gesture, NMnist, and Cifar10-DVS datasets (see~\autoref{tab:prune_defense}). As can be seen, even though the initial clean accuracy and ASR are high before pruning, we observe a substantial decrease in the clean accuracy across all datasets (except on NMnist, where the drop is less noticeable) after pruning.

% In general, we observe that the defense has little effect when pruning this amount of neurons on the DVS128-Gesture dataset, and there are no meaningful differences in the defense performance between different trigger lengths or attacks, resulting in a significant decrease in the clean accuracy with little to no effect on the ASR. We observe similar outcomes on the NMnist dataset; however, the defense's efficacy in this dataset exhibited a notably higher level of variability across different runs.

% Finally, on the Cifar10-DVS dataset, the defense is quite effective against the smaller-sized triggers. However, this defense can not remove the backdoor behavior when a flash trigger is present. It is important to note that after applying this defense, the general clean accuracy plummeted from around  65\% to a mere 15\%, meaning that if the user applied this defense on their model, they would have lost all the model's performance.

% On the other hand, the inclusion of the strobing trigger led to a more unpredictable performance of this defense mechanism for all the tested datasets, making it harder to be reliably removed. 

% However, a general tendency can be observed in the results, as pruned models trained with bigger triggers tend to have a more substantial drop in the clean accuracy and less impact on the ASR. These results were to be expected; a smaller trigger can be more discreet, but it also has a lesser impact on the model, mainly injecting the backdoor on less influential neurons. The pruning process first focuses on removing these less influential neurons, making it easier to erase the backdoor behavior. However, with the introduction of larger triggers, their influence on the model is also amplified, making them more challenging to target through pruning.

% When applying this procedure to the selected model for real-world environments, we observe results similar to those obtained in digital scenarios. The model suffers from an even bigger drop in the clean accuracy, going from 73.03\% to 8.98\% with no variation between experiments; this suggests that the model's performance is less stable with newly-captured samples, it is to be expected, as our samples do not perfectly match the ones from the original DVS128-Gesture dataset and there has not been any fine-tunning to adapt the model to our samples. On the other hand, the ASR does not show any change, maintaining 100\% of effectivity, suggesting that the triggers are robust enough against changes, as our triggers do not fit the digital ones perfectly either. In conclusion, the pruning procedure is not able to reliably remove the backdoor by itself, neither in digital or real-world environments, even when sacrificing most of the clean accuracy of the model.

% We also conduct an evaluation of the influence the pruning rate has on the clean accuracy and the ASR of the selected model to transfer the attack onto physical environments, increasing this parameter in steps of 10\% from 10\% to 90\%. And, as shown in~\autoref{tab:prune_steps}, increasing the running rate gradually decreases the clean accuracy but does not influence the ASR, suggesting that the pruned neurons do not contain the backdoor behavior, making this procedure ineffective against this particular attack method.

% \begin{table}[ht]
% \centering
% \caption{Evaluation of the effect of the pruning rate on the clean accuracy and the ASR of the model trained for 80 epochs with a trigger with polarity $p=3$ a size of 10\% of the original image situated at the beginning of the sample.}
% \begin{tabular}{@{}ccccc@{}}
% \toprule
% \textbf{$\tau$} & \textbf{I\_CA} & \textbf{I\_ASR} & \textbf{Pruned\_CA} & \textbf{Pruned\_ASR} \\ \midrule
% 0.1 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 88.54 $\pm$ 2.46 & 99.83 $\pm$ 0.25 \\
% 0.2 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 86.63 $\pm$ 5.16 & 100 $\pm$ 0.0 \\
% 0.3 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 79.86 $\pm$ 12.77 & 100 $\pm$ 0.0 \\
% 0.4 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 68.58 $\pm$ 20.38 & 100 $\pm$ 0.0 \\
% 0.5 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 48.09 $\pm$ 20.87 & 100 $\pm$ 0.0 \\
% 0.6 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 30.03 $\pm$ 17.92 & 100 $\pm$ 0.0 \\
% 0.7 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 17.19 $\pm$ 12.52 & 100 $\pm$ 0.0 \\
% 0.8 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 11.63 $\pm$ 4.66 & 100 $\pm$ 0.0 \\
% 0.9 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 8.68 $\pm$ 0.49 & 100 $\pm$ 0.0 \\ \bottomrule
% \end{tabular}
% \label{tab:prune_steps}
% \end{table}


\subsubsection{Fine-tuning}
\label{tab:prune_defense}
In general, fine-tuning refers to taking a pre-trained neural network model and further training it on a new dataset or task. The pre-trained model is typically initialized with weights learned from training on a large, general dataset. During fine-tuning, the parameters of the pre-trained model are adjusted or fine-tuned to adapt to the specifics of the new dataset or task. This adjustment allows the model to learn task-specific features and patterns while leveraging the knowledge captured by the pre-trained model. 

In our case, we take the given backdoored model and retrain it for a fixed amount of epochs on a clean dataset, allowing the model to try to ``forget'' the backdoor behavior. This is based on the concept of ``catastrophic forgetting'', which refers to the phenomenon where a neural network model trained on a specific task or dataset forgets previously learned information when trained on a new task or dataset~\cite{forgetting}.

We fine-tune the model for 10\% of the network's original training epochs with the clean DVS128-Gesture, NMnist, and Cifar10-DVS datasets, focusing again on each attack type's trigger length and size (see~\autoref{tab:tune_defense}). This decision was taken based on the threat model, as the user who requested the service would not have the resources needed for extensive training. 


\begin{table*}[ht]
\centering
\caption{Results of the fine-tuning procedure with the number of tuning epochs set to 10\% of the original amount, the model was trained for all the presented attacks and the DVS128-Gesture, NMnist, and Cifar10-DVS datasets.}
\resizebox{\textwidth}{!}{ % adjust margins
\begin{tabular}{@{}ccccccccc@{}}
\cmidrule(r){1-9}
\textbf{Dataset} & \textbf{Size} & \textbf{Attack} & \textbf{P Frames} & \textbf{Ini CA\%} & \textbf{I\_ASR\%} & \textbf{FT epochs} & \textbf{FT CA\%} & \textbf{FT ASR\%}\\ \cmidrule(r){1-9}
DVS128-Gesture & 0.3 & Static & 16 & 90.62 $\pm$ 0.35 & 99.08 $\pm$ 0.40        & 4 & 88.08 $\pm$ 2.12 & 68.98 $\pm$ 7.29 \\
DVS128-Gesture & 0.3 & Framed & 12 & 91.20 $\pm$ 1.00 & 99.08 $\pm$ 0.20        & 4 & 89.70 $\pm$ 1.64 & 70.25  $\pm$ 5.95 \\
DVS128-Gesture & 0.3 & Framed & 6 & 89.47 $\pm$ 1.56 & 54.63 $\pm$ 35.50        & 4 & 85.88 $\pm$ 5.23 & 14.59  $\pm$ 3.31 \\
DVS128-Gesture & 0.3 & Strobing & 6 & 89.00 $\pm$ 1.56 & 97.80 $\pm$ 0.87       & 4 & 87.15 $\pm$ 3.62 & 21.30  $\pm$ 16.47  \\
DVS128-Gesture & 1 & Flash & 6 & 90.20 $\pm$ 0.92 & 99.54 $\pm$ 0.53            & 4 & 86.34 $\pm$ 2.63 & 47.22  $\pm$ 19.95  \\
DVS128-Gesture & 1 & Flash & 3 & 87.61 $\pm$ 1.91 & 96.64 $\pm$ 4.07            & 4 & 87.62 $\pm$ 0.87 & 15.63  $\pm$ 5.46 \\
DVS128-Gesture & 1 & Strobing Flash & 3 & 88.31 $\pm$ 2.81 & 90.28 $\pm$ 15.04  & 4 & 89.46 $\pm$ 1.22 &  23.61 $\pm$ 12.28 \\ \cmidrule(r){1-9}
NMnist & 0.3 & Static & 16 & 99.28 $\pm$ 0.03 & 99.97 $\pm$ 0.00                & 2 & 99.05 $\pm$ 0.12 &  99.93 $\pm$ 0.07  \\
NMnist & 0.3 & Framed & 10 & 99.28 $\pm$ 0.03 & 99.97 $\pm$ 0.00                & 2 & 99.08 $\pm$ 0.11 &  99.97 $\pm$ 0.01  \\
NMnist & 0.3 & Framed & 5 & 99.24 $\pm$ 0.03 & 99.97 $\pm$ 0.01                 & 2 & 99.19 $\pm$ 0.03 &  99.97 $\pm$ 0.07  \\
NMnist & 0.3 & Strobing & 5 & 99.29 $\pm$ 0.04 & 99.97 $\pm$ 0.01               & 2 & 99.01 $\pm$ 0.15 &  99.83 $\pm$ 0.25  \\
NMnist & 1 & Flash & 6 & 99.29 $\pm$ 0.03 & 99.97 $\pm$ 0.02                    & 2 & 99.05 $\pm$ 0.07 &  99.96 $\pm$ 0.01  \\
NMnist & 1 & Flash & 3 & 99.27 $\pm$ 0.02 & 99.97 $\pm$ 0.00                    & 2 & 99.01 $\pm$ 0.08 &  99.97 $\pm$ 0.01 \\
NMnist & 1 & Strobing Flash & 3 & 99.30 $\pm$ 0.02 & 99.96 $\pm$ 0.01           & 2 & 99.02 $\pm$ 0.23 &  99.95 $\pm$ 0.06  \\ \cmidrule(r){1-9}
Cifar10-DVS & 0.3 & Static & 16 & 67.47 $\pm$ 0.78 & 95.83 $\pm$ 0.06           & 2 & 65.93 $\pm$ 0.95 &  85.30 $\pm$ 2.43  \\
Cifar10-DVS & 0.3 & Framed & 10 & 67.30 $\pm$ 0.90 & 95.67 $\pm$ 0.06           & 2 & 66.13 $\pm$ 0.85 &  90.87 $\pm$ 6.20 \\
Cifar10-DVS & 0.3 & Framed & 5 & 66.33 $\pm$ 0.61 & 95.60 $\pm$ 0.10            & 2 & 64.37 $\pm$ 1.02 &  87.63 $\pm$ 6.55 \\
Cifar10-DVS & 0.3 & Strobing & 5 & 66.20 $\pm$ 0.72 & 95.57 $\pm$ 0.21          & 2 & 64.30 $\pm$ 1.54 &  95.23 $\pm$ 2.51  \\
Cifar10-DVS & 1 & Flash & 6 & 63.40 $\pm$ 0.98 & 95.87 $\pm$ 0.15               & 2 & 61.67 $\pm$ 1.47 &  95.40 $\pm$ 0.17 \\
Cifar10-DVS & 1 & Flash & 3 & 63.97 $\pm$ 0.93 & 95.57 $\pm$ 0.42               & 2 & 62.77 $\pm$ 1.00 &  85.90 $\pm$ 9.01 \\
Cifar10-DVS & 1 & Strobing Flash & 3 & 64.47 $\pm$ 1.12 & 95.53 $\pm$ 0.21      & 2 & 61.63 $\pm$ 1.80 &  95.80 $\pm$ 0.26 \\ \cmidrule(r){1-9}
\end{tabular}
}
\label{tab:tune_defense}
\end{table*}

% \begin{table*}[ht]
% \centering
% \caption{Results of the fine-tuning defense: With the number of tuning epochs set to 10\% of the original amount, the model was trained for all the presented attacks in the DVS128-Gesture, NMnist, and Cifar10-DVS datasets.}
% \resizebox{\textwidth}{!}{ % adjust margins
% \begin{tabular}{@{}ccccccccc@{}}
% \cmidrule(r){1-9}
% \textbf{Dataset} & \textbf{Size} & \textbf{Attack} & \textbf{P Frames} & \textbf{Ini CA\%} & \textbf{I\_ASR\%} & \textbf{FT epochs} & \textbf{FT CA\%} & \textbf{FT ASR\%}\\ \cmidrule(r){1-9}
% DVS128-Gesture & 0.3 & Static & 16 & 92.71& 99.31& 4 & 92.36 $\pm$ 0.01 & 99.31 $\pm$ 1.36E-16 \\
% DVS128-Gesture & 0.3 & Framed & 12 & 92.36& 99.31& 4 & 92.25 $\pm$ 0.01 & 99.31 $\pm$ 3.47E-03 \\
% DVS128-Gesture & 0.3 & Framed & 6 & 91.67& 99.42& 4 & 90.74 $\pm$ 0.01 & 99.19 $\pm$ 5.30E-03 \\
% DVS128-Gesture & 0.3 & Strobing & 6 & 92.01& 99.31& 4 & 92.25 $\pm$ 0.0 & 99.42 $\pm$ 2.00E-03 \\
% DVS128-Gesture & 1 & Flash & 6 & 92.71& 99.42& 4 & 92.59 $\pm$ 0.0 & 99.07 $\pm$ 2.00E-03 \\
% DVS128-Gesture & 1 & Flash & 3 & 91.90& 98.96& 4 & 90.97 $\pm$ 0.01 & 98.96 $\pm$ 3.47E-03 \\
% DVS128-Gesture & 1 & Strobing Flash & 3 & 88.19& 99.65& 4 & 92.01 $\pm$ 0.0& 99.42 $\pm$ 5.30E-03 \\ \cmidrule(r){1-9}
% NMnist & 0.3 & Static & 16 & 99.49& 99.98& 2 & 99.46 $\pm$ 0.0 & 99.98 $\pm$ 1.15E-04 \\
% NMnist & 0.3 & Framed & 10 & 99.46& 99.98& 2 & 99.48 $\pm$ 0.0 & 99.98 $\pm$ 5.77E-05 \\
% NMnist & 0.3 & Framed & 5 & 99.42& 99.97& 2 & 99.44 $\pm$ 0.0 & 99.97 $\pm$ 5.77E-05 \\
% NMnist & 0.3 & Strobing & 5 & 99.46& 99.98& 2 & 99.48 $\pm$ 0.0 & 99.98 $\pm$ 5.77E-05 \\
% NMnist & 1 & Flash & 6 & 99.47& 99.97& 2 & 99.47 $\pm$ 0.0 & 99.98 $\pm$ 1.00E-04 \\
% NMnist & 1 & Flash & 3 & 99.44& 99.98& 2 & 99.44 $\pm$ 0.0 & 99.98 $\pm$ 0.0 \\
% NMnist & 1 & Strobing Flash & 3 & 99.44& 99.98& 2 & 99.42 $\pm$ 0.0 & 99.98 $\pm$ 5.77E-05 \\ \cmidrule(r){1-9}
% Cifar10-DVS & 0.3 & Static & 16 & 67.57& 95.57& 2 & 67.53 $\pm$ 0.0 & 95.63 $\pm$ 2.52E-03 \\
% Cifar10-DVS & 0.3 & Framed & 10 & 67.87& 95.67& 2 & 67.73 $\pm$ 0.01 & 95.57 $\pm$ 4.93E-03 \\
% Cifar10-DVS & 0.3 & Framed & 5 & 67.10& 95.43& 2 & 66.67 $\pm$ 0.01 & 95.50 $\pm$ 3.00E-03 \\
% Cifar10-DVS & 0.3 & Strobing & 5 & 67.17& 95.80& 2 & 67.20 $\pm$ 0.0 & 95.63 $\pm$ 4.51E-03 \\
% Cifar10-DVS & 1 & Flash & 6 & 65.10& 96.27& 2 & 65.27 $\pm$ 0.01 & 96.23 $\pm$ 4.16E-03 \\
% Cifar10-DVS & 1 & Flash & 3 & 63.07& 96.37& 2 & 64.33 $\pm$ 0.01 & 96.40 $\pm$ 6.00E-03 \\
% Cifar10-DVS & 1 & Strobing Flash & 3 & 65.70& 96.23& 2 & 65.10 $\pm$ 0.01 & 95.53 $\pm$ 3.79E-03 \\ \cmidrule(r){1-9}
% Real-samples & 1 & Strobing Flash & 2 & 73.03& 100& 8 & 66.66 $\pm$ 5.07 & 95.72 $\pm$ 7.40 \\ \cmidrule(r){1-9}
% \end{tabular}
% }
% \label{tab:tune_defense}
% \end{table*}


For the DVS128-Gesture dataset, the fine-tuning procedure demonstrates partial effectiveness. We observe a significant reduction in ASR after fine-tuning for attacks with smaller trigger sizes and shorter trigger lengths. For example, in the Strobing attack with a trigger of 30\% and six poisoned frames, ASR drops more than 70\% while the clean accuracy only decreases by 2\%. However, for attacks containing larger trigger sizes or longer poisoned sequences, the procedure is less effective; if we compare the Flash attack with the same number of poisoned frames, the ASR reduction was 26\% less effective.

In the case of the NMnist dataset, the fine-tuning procedure proves largely ineffective. The ASR remains high after fine-tuning, often above 99\%, regardless of the trigger length or size. This suggests that a brief period of fine-tuning is insufficient to mitigate the attack. We can also see similar results for the Cifar10-DVS dataset; the fine-tuning procedure results in modest reductions in ASR, but despite the reduction, ASR remains above 85\%, suggesting that the backdoor is not effectively removed.

Our results suggest that fine-tuning the models for this amount of epochs can reduce the backdoor effect for certain datasets and attack configurations, particularly those involving smaller triggers and shorter trigger lengths on the DVS128-Gesture dataset. However, longer triggers and larger trigger sizes tend to be more resilient, showing less reduction in ASR after fine-tuning. It is also noteworthy that including a clean frame between triggers resulted in higher ASRs across all tested datasets than their continuous counterparts. 


% When applying this procedure to the model selected for real-world environments, we observe a slight reduction in the clean accuracy; we hypothesize that due to the model partially losing its capacity to generalize on samples different from the ones of the original dataset it was trained on, caused by a small over-fitting. On the other hand, we see a more significant drop in the ASR with a reduction of 4.28\%. When comparing it to the results obtained in its digital counterpart, it suggests that the ability of the backdoor behavior to generalize to slight differences in the triggers is partially lost when fine-tuning the model. Thus, we theorize that it could possibly be reduced even further with a larger amount of fine-tuning epochs. However, we cannot affirm that it is able to eliminate the backdoor behavior in either environment, at least not with the limited processing power imposed by the threat model. Additionally, we can also observe that the variance of these results is much higher than that obtained with digital samples, thus making the application of this defense more unreliable in this scenario.


\subsubsection{Fine-pruning}
This defense~\cite{fine_prune} is a combination of both pruning and fine-tuning. The defender first prunes the network and then fine-tunes the result. The main intuition behind this defense is that the initial pruning removes the backdoor neurons, and the following fine-tuning restores the drop in classification accuracy on the clean inputs introduced by the pruning. Even if this defense can be effective when the trigger size is small, as demonstrated by Abad et al.~\cite{paperGorka2}, when applied against larger triggers, the results are not straightforward. We can observe a higher success when comparing to the previous two methods, achieving a substantial reduction in ASR, albeit with a high impact on the clean accuracy (see~\autoref{tab:fine_prune_defense}). We can conclude that the pruning of the lower mean activation neurons enabled the fine-tuning to focus on the backdoor-containing ones, but we observe a similar tendency as in the fine-tuning method; the epochs used to retrain the model are not sufficient to recover the clean accuracy nor to completely erase the backdoor behavior.\todo{then, why not more epochs? R:find paper and add it}

% Similar to the fine-tuning defense, the inclusion of a clean frame between triggers resulted in higher and more stable ASR in both DVS128-Gesture and Cifar10-DVS datasets when compared to their continuous version. However, this time, the clean accuracy suffered more in some cases, suggesting it could be more challenging to recover the clean accuracy lost during the pruning phase with fine-tuning when the trigger is not continuous.

% When applying this defense to the model selected for real-world environments, we observe similar results to the ones obtained in digital scenarios. While the fine-tuning epochs after the running can recover some of the clean accuracy, those are not sufficient to return to its original state. We also observe that the reduction of the ASR is higher than the one obtained by merely fine-tuning the model. This could be attributed to the pruning applied to the less influential neurons, as this enables the model to focus on the training of the unpruned, more influential neurons, where the backdoor is mainly contained. However, we can also see an increase in the variability of the results, suggesting that reducing the number of neurons to be tuned increases the susceptibility of the training procedure to slight changes.

% Consequently, after seeing the results and considering the threat model's limitations, we can not affirm that this defense is able to reliably remove the backdoor from a corrupted model in either digital or physical environments.


For the DVS128-Gesture dataset, the fine-pruning defense is effective across all attack types and trigger configurations. After applying the defense, we observe a significant reduction in ASR while maintaining most of the clean accuracy. 
In the case of the NMnist dataset, the fine-pruning defense shows partial effectiveness. While the clean accuracy remains high after the defense, ASR decreases significantly for attacks with smaller shorter triggers. However, for attacks with larger or longer\todo{?}, ASR remains relatively high, indicating that the backdoor is not entirely mitigated. 
For the Cifar10-DVS dataset, the fine-pruning defense yields mixed results. It is more effective against attacks with smaller trigger sizes and longer poisoned frame sequences, where we observe a substantial reduction in ASR and minimal impact on clean accuracy. However, for attacks involving larger trigger sizes or shorter poisoned sequences, ASR remains relatively high after fine-pruning.

We hypothesize that the reason this defense performs better than fine-tuning alone, even though pruning by itself does not seem to be effective, is that pruning the less important neurons allows the fine-tuning process to focus on the more critical neurons where the backdoor is embedded. By eliminating the neurons that contribute least to the model's overall performance, fine-pruning reduces the model's capacity to retain the backdoor behavior. This targeted approach enables the fine-tuning phase to overwrite the backdoor-influenced parameters, thus enhancing the defense's effectiveness.

% In conclusion, the fine-pruning defense offers a more robust strategy for mitigating backdoor attacks compared to fine-tuning or pruning alone. And, although it shows potential by significantly reducing the ASR in some scenarios, we cannot state that it is an effective defense across all datasets and attack configurations.

It is also to be noted that fine-pruning focuses on identifying and nullifying the model parameters that introduce the malicious behavior. However, as demonstrated in previous works~\cite{paperGorka2}, when faced with an adaptive attacker, it becomes easily evaded. As discussed by Abad et al.~\cite{paperGorka2}, an attacker who knows that the last convolutional layer is targeted for pruning could just limit the backdoor injection to the rest of the network or reduce the poisoning rate, achieving high ASR and nullify the pruning procedure.

\begin{table*}[ht]
\centering
\caption{Results of the fine-pruning defense: With a pruning rate of 0.8 and the number of tuning epochs set to 10\% of the original amount the model was trained for all the presented attacks and the DVS128-Gesture, NMnist, and Cifar10-DVS datasets.}\todo{?}
\resizebox{\textwidth}{!}{ % adjust margins
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Size} & \textbf{Attack} & \textbf{P Frames} & \textbf{Ini CA\%} & \textbf{I\_ASR\%} & \textbf{$\tau$} & \textbf{FT epochs} & \textbf{FP CA\%} & \textbf{FP ASR\%} \\ \midrule
DVS128-Gesture & 0.3 & Static & 16 & 90.62 $\pm$ 0.35 & 99.08 $\pm$ 0.40        & 0.8 & 4 & 86.34 $\pm$ 1.75 & 17.71 $\pm$ 3.63 \\
DVS128-Gesture & 0.3 & Framed & 12 & 91.20 $\pm$ 1.00 & 99.08 $\pm$ 0.20        & 0.8 & 4 & 90.74 $\pm$ 2.44 & 21.99 $\pm$ 1.56 \\
DVS128-Gesture & 0.3 & Framed & 6 & 89.47 $\pm$ 1.56 & 54.63 $\pm$ 35.50        & 0.8 & 4 & 87.96 $\pm$ 3.11 & 10.19 $\pm$ 2.26 \\
DVS128-Gesture & 0.3 & Strobing & 6 & 89.00 $\pm$ 1.56 & 97.80 $\pm$ 0.87       & 0.8 & 4 & 89.47 $\pm$ 1.71 & 11.11 $\pm$ 4.52 \\
DVS128-Gesture & 1 & Flash & 6 & 90.20 $\pm$ 0.92 & 99.54 $\pm$ 0.53            & 0.8 & 4 & 86.80 $\pm$ 3.31 & 14.82 $\pm$ 4.18 \\
DVS128-Gesture & 1 & Flash & 3 & 87.61 $\pm$ 1.91 & 96.64 $\pm$ 4.07            & 0.8 & 4 & 81.25 $\pm$ 1.59 & 8.68 $\pm$ 1.39 \\
DVS128-Gesture & 1 & Strobing Flash & 3 & 88.31 $\pm$ 2.81 & 90.28 $\pm$ 15.04  & 0.8 & 4 & 87.50 $\pm$ 2.84 & 8.45 $\pm$ 1.11 \\ \midrule
NMnist & 0.3 & Static & 16 & 99.28 $\pm$ 0.03 & 99.97 $\pm$ 0.00                & 0.8 & 2 & 98.81 $\pm$ 0.12 & 32.99 $\pm$ 15.03 \\
NMnist & 0.3 & Framed & 10 & 99.28 $\pm$ 0.03 & 99.97 $\pm$ 0.00                & 0.8 & 2 & 98.72 $\pm$ 0.25 & 28.42 $\pm$ 15.73 \\
NMnist & 0.3 & Framed & 5 & 99.24 $\pm$ 0.03 & 99.97 $\pm$ 0.01                 & 0.8 & 2 & 98.80 $\pm$ 0.13 & 21.84 $\pm$ 2.56 \\
NMnist & 0.3 & Strobing & 5 & 99.29 $\pm$ 0.04 & 99.97 $\pm$ 0.01               & 0.8 & 2 & 98.83 $\pm$ 0.08 & 49.01 $\pm$ 23.06 \\
NMnist & 1 & Flash & 6 & 99.29 $\pm$ 0.03 & 99.97 $\pm$ 0.02                    & 0.8 & 2 & 98.74 $\pm$ 0.16 & 99.95 $\pm$ 0.04 \\
NMnist & 1 & Flash & 3 & 99.27 $\pm$ 0.02 & 99.97 $\pm$ 0.00                    & 0.8 & 2 & 98.87 $\pm$ 0.06 & 83.45 $\pm$ 20.19\\
NMnist & 1 & Strobing Flash & 3 & 99.30 $\pm$ 0.02 & 99.96 $\pm$ 0.01           & 0.8 & 2 & 98.82 $\pm$ 0.13 & 60.95 $\pm$ 40.13 \\ \midrule
Cifar10-DVS & 0.3 & Static & 16 & 67.47 $\pm$ 0.78 & 95.83 $\pm$ 0.06           & 0.8 & 2 & 65.20 $\pm$ 1.51 & 29.43 $\pm$ 13.31\\
Cifar10-DVS & 0.3 & Framed & 10 & 67.30 $\pm$ 0.90 & 95.67 $\pm$ 0.06           & 0.8 & 2 & 65.23 $\pm$ 1.52 & 56.57 $\pm$ 12.68 \\
Cifar10-DVS & 0.3 & Framed & 5 & 66.33 $\pm$ 0.61 & 95.60 $\pm$ 0.10            & 0.8 & 2 & 62.70 $\pm$ 3.05 & 64.83 $\pm$ 5.18 \\
Cifar10-DVS & 0.3 & Strobing & 5 & 66.20 $\pm$ 0.72 & 95.57 $\pm$ 0.21          & 0.8 & 2 & 63.67 $\pm$ 1.16 & 95.40 $\pm$ 0.89 \\
Cifar10-DVS & 1 & Flash & 6 & 63.40 $\pm$ 0.98 & 95.87 $\pm$ 0.15               & 0.8 & 2 & 63.03 $\pm$ 1.16 & 95.40 $\pm$ 0.89 \\
Cifar10-DVS & 1 & Flash & 3 & 63.97 $\pm$ 0.93 & 95.57 $\pm$ 0.42               & 0.8 & 2 & 61.60 $\pm$ 0.17 & 55.73 $\pm$ 10.23 \\
Cifar10-DVS & 1 & Strobing Flash & 3 & 64.47 $\pm$ 1.12 & 95.53 $\pm$ 0.21      & 0.8 & 2 & 63.70 $\pm$ 0.85 & 92.30 $\pm$ 4.16 \\ \bottomrule
\end{tabular}
}
\label{tab:fine_prune_defense}
\end{table*}
% \begin{table*}[ht]
% \centering
% \caption{Results of the fine-pruning defense: With a pruning rate of 0.8 and the number of tuning epochs set to 10\% of the original amount the model was trained for all the presented attacks in the DVS128-Gesture, NMnist, and Cifar10-DVS datasets.}
% \resizebox{\textwidth}{!}{ % adjust margins
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% \textbf{Dataset} & \textbf{Size} & \textbf{Attack} & \textbf{P Frames} & \textbf{Ini CA\%} & \textbf{I\_ASR\%} & \textbf{$\tau$} & \textbf{FT epochs} & \textbf{FP CA\%} & \textbf{FP ASR\%} \\ \midrule
% DVS128-Gesture & 0.3 & Static & 16 & 92.71& 99.31               & 0.8 & 4 & 47.80 $\pm$ 0.02 & 86.11 $\pm$ 0.20 \\
% DVS128-Gesture & 0.3 & Framed & 12 & 92.36& 99.31               & 0.8 & 4 & 53.94 $\pm$ 0.03 & 64.58 $\pm$ 0.27 \\
% DVS128-Gesture & 0.3 & Framed & 6 & 91.67& 99.42                & 0.8 & 4 & 47.80 $\pm$ 0.08 & 54.17 $\pm$ 0.03 \\
% DVS128-Gesture & 0.3 & Strobing & 6 & 92.01& 99.31              & 0.8 & 4 & 48.50 $\pm$ 0.07 & 76.85 $\pm$ 0.17 \\
% DVS128-Gesture & 1 & Flash & 6 & 92.71& 99.42                   & 0.8 & 4 & 56.48 $\pm$ 0.01 & 70.02 $\pm$ 0.51 \\
% DVS128-Gesture & 1 & Flash & 3 & 91.90& 98.96                   & 0.8 & 4 & 60.65 $\pm$ 0.18 & 42.59 $\pm$ 0.27 \\
% DVS128-Gesture & 1 & Strobing Flash & 3 & 88.19& 99.65          & 0.8 & 4 & 26.16 $\pm$ 0.11 & 93.87 $\pm$ 0.11 \\ \midrule
% NMnist & 0.3 & Static & 16 & 99.49& 99.98                       & 0.8 & 2 & 93.84 $\pm$ 0.03 & 99.91 $\pm$ 0.0 \\
% NMnist & 0.3 & Framed & 10 & 99.46& 99.98                       & 0.8 & 2 & 96.80 $\pm$ .0.0 & 96.16 $\pm$ 0.07 \\
% NMnist & 0.3 & Framed & 5 & 99.42& 99.97                        & 0.8 & 2 & 96.43 $\pm$ 0.01 & 93.71 $\pm$ 0.07 \\
% NMnist & 0.3 & Strobing & 5 & 99.46& 99.98                      & 0.8 & 2 & 95.97 $\pm$ 0.03 & 69.64 $\pm$ 0.51 \\
% NMnist & 1 & Flash & 6 & 99.47& 99.97                           & 0.8 & 2 & 97.04 $\pm$ 0.01 & 71.24 $\pm$ 0.49 \\
% NMnist & 1 & Flash & 3 & 99.44& 99.98                           & 0.8 & 2 & 94.12 $\pm$ 0.05 & 99.74 $\pm$ 0.0 \\
% NMnist & 1 & Strobing Flash & 3 & 99.44& 99.98                  & 0.8 & 2 & 94.37 $\pm$ 0.02 & 49.85 $\pm$ 0.44 \\ \midrule
% Cifar10-DVS & 0.3 & Static & 16 & 67.57& 95.57                  & 0.8 & 2 & 44.70 $\pm$ 0.01 & 95.93 $\pm$ 0.0 \\
% Cifar10-DVS & 0.3 & Framed & 10 & 67.87& 95.67                  & 0.8 & 2 & 38.77 $\pm$ 0.10 & 75.87 $\pm$ 0.28 \\
% Cifar10-DVS & 0.3 & Framed & 5 & 67.10& 95.43                   & 0.8 & 2 & 38.27 $\pm$ 0.04 & 90.00 $\pm$ 0.07 \\
% Cifar10-DVS & 0.3 & Strobing & 5 & 67.17& 95.80                 & 0.8 & 2 & 38.90 $\pm$ 0.03 & 76.97 $\pm$ 0.32 \\
% Cifar10-DVS & 1 & Flash & 6 & 65.10& 96.27                      & 0.8 & 2 & 39.07 $\pm$ 0.07 & 59.13 $\pm$ 0.48 \\
% Cifar10-DVS & 1 & Flash & 3 & 63.07& 96.37                      & 0.8 & 2 & 35.73 $\pm$ 0.03 & 86.70 $\pm$ 0.07 \\
% Cifar10-DVS & 1 & Strobing Flash & 3 & 65.70& 96.23             & 0.8 & 2 & 33.00 $\pm$ 0.02 & 92.67 $\pm$ 0.01 \\ \bottomrule
% \end{tabular}
% }
% \label{tab:fine_prune_defense}
% \end{table*}

% We proceed with a similar evaluation to the one we did on the pruning procedure, increasing the pruning rate in steps of 10\% to test its influence, while also observing if the model is able to recover the lost clean accuracy with the subsequent training. As can be seen in~\autoref{tab:fineprune_steps}, it produced close results to the ones obtained with just the pruning procedure~\autoref{tab:prune_steps}, the ASR is not affected at all. However, unlike applying just the pruning, the model is able to mostly recover its lost clean accuracy when the pruning rate is low. Thus, we conclude that the defense is not effective against our attack as neither the pruning nor the subsequent pruning are able to eliminate the backdoor behavior.


%  \begin{table}[ht]
% \centering
% \caption{Evaluation of the effect of the pruning rate fine-prune defense with 8 fine-tunning epochs on the clean accuracy and the ASR of the model trained for 80 epochs, with a trigger with polarity $p=3$ a size of 10\% of the original image situated at the beginning of the sample.}
% \begin{tabular}{@{}cccll@{}}
% \toprule
% \textbf{$\tau$} & \textbf{I CA} & \textbf{I ASR} & \multicolumn{1}{c}{\textbf{FP CA}} & \multicolumn{1}{c}{\textbf{FP ASR}} \\ \midrule
% 0.1 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 90.80 $\pm$ 0.74 & 98.96 $\pm$ 0.49 \\
% 0.2 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 90.80 $\pm$ 0.25 & 99.31 $\pm$ 0.98 \\
% 0.3 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 89.58 $\pm$ 1.47 & 99.48 $\pm$ 0.74 \\
% 0.4 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 86.11 $\pm$ 5.89 & 99.65 $\pm$ 0.49 \\
% 0.5 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 73.09 $\pm$ 18.41 & 99.83 $\pm$ 0.25 \\
% 0.6 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 60.24 $\pm$ 26.76 & 99.83 $\pm$ 0.25 \\
% 0.7 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 51.56 $\pm$ 37.07 & 100 $\pm$ 0.0 \\
% 0.8 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 40.63 $\pm$ 31.92 & 99.83 $\pm$ 0.25 \\
% 0.9 & 90.79 $\pm$ 0.06 & 99.13 $\pm$ 0.73 & 14.93 $\pm$ 7.86 & 100 $\pm$ 0.0 \\ \bottomrule
% \end{tabular}
% \label{tab:fineprune_steps}
% \end{table}


\subsection{Evaluation of the Stealthiness}

Assessing the stealthiness of triggers in backdoor attacks is critical to ensure their effectiveness while remaining undetected. In practical applications, the datasets employed are often extensive~\cite{VeryBigData}, making it impractical to visually evaluate the presence of triggers by human users. Manual inspection would be not only time-consuming~\cite{BigDataTimeConsuming} but also prone to human error and subjectivity~\cite{humanError}, making it an inefficient method for large-scale datasets as it happens with datasets containing missing samples~\cite{LargeScale}.\todo{?}

To address this challenge, quantitative metrics are utilized to objectively evaluate the imperceptibility of the backdoor triggers. These metrics provide a systematic approach to measure the similarity between the original, unaltered images and the images containing the backdoor triggers, ensuring that the triggers are not easily detectable by users or automated systems. Some of the commonly used metrics are the Mean Squared Error (MSE), the Structural Similarity Index Measure (SSIM), and the Peak Signal-to-Noise Ratio (PSNR)~\cite{common_metrics}. We additionally propose an entropy evaluation of the activation values, the number of activations across a whole frame, and the entropy on those same amounts among each frame.\todo{?} 
%Refer to~\autoref{appendixC} for additional explored detection mechanisms and experiments.


\subsubsection{Mean Squared Error}
The MSE~\cite{mse} metric calculates the average square values of the differences between the corresponding pixel values of the original and the modified images. Formally: 
$$\text{MSE} = \frac{1}{N} \sum_{i=1}^N (\textbf{a}_i - \textbf{b}_i)^2,$$
where $\textbf{a}_i$ is the pixel value of the original image,  $\textbf{b}_i$ is the pixel value of the triggered image, and $N$ is the total number of pixels. A lower MSE value indicates higher similarity between the images, suggesting that the trigger is less perceptible. However, this metric is discussed not to be a good representation of how a human user would discern the change in the image~\cite{mse}, as it does not take into account the context of the neighboring pixels. This metric would give the same result for a change of 10\% of the total pixel amount distributed across the image or all of them focused on the same spot, resulting in an evident change for a human user but resulting in the same MSE.

\subsubsection{Structural Similarity Index Measure}

SSIM, proposed by Wang et al.~\cite{ssim}, is another widely used metric that assesses the visual impact of changes in structural information between two images~\cite{common_metrics}. Unlike MSE, SSIM considers luminance, contrast, and structure changes, making it more aligned with human visual perception. The SSIM index ranges from -1 to 1, where 1 indicates perfect structural similarity. The SSIM is calculated as:
$$\text{SSIM}(\textbf{a}, \textbf{b}) = \frac{(2\mu_a \mu_b + C_1)(2\sigma_{ab} + C_2)}{(\mu_a^2 + \mu_b^2 + C_1)(\sigma_a^2 + \sigma_b^2 + C_2)},
$$
where $\mu_a$ and $\mu_b$ are the average pixel values of the original and triggered images, $\sigma_a^2$ and $\sigma_b^2$ are the variances, and $\sigma_{ab}$ is the covariance of the images. $C_1$ and $C_2$ are constants to stabilize the division.

\subsubsection{Peak Signal-to-Noise Ratio}

PSNR is a commonly used metric to evaluate the quality of an image by comparing the original and the altered image~\cite{psnr}. Opposed to the MSE metric, it takes into account images having different dynamic ranges~\cite{mse}, which in this case can be very beneficial since the pixels have no set range; it depends on the number of activations that occurred on the selected time frame. This metric expresses the ratio between the maximum possible power of a signal and the power of corrupting noise that affects the fidelity of its representation. PSNR is expressed in decibels (dB) and is inversely related to the MSE. Formally:
$$\text{PSNR} = 10 \cdot \log_{10} \left(\frac{\text{MAX}^2}{\text{MSE}}\right),$$
where $\text{MAX}$ is the maximum possible pixel value of the image. A higher PSNR value indicates that the differences between the original and the triggered images are less perceptible.

PSNR is particularly useful in scenarios where the human perception of image quality is crucial. It is extensively used in image compression, transmission, and processing to evaluate how much an image has been degraded by these processes~\cite{psnr}. In the context of backdoor attacks, a high PSNR value would suggest that the trigger is well-hidden and does not significantly degrade the image quality, thus remaining stealthy.

\subsubsection{Entropy of the Activation Values}

Entropy measures the amount of randomness in the pixel values of an image. Lower entropy values in the trigger image, when compared to the base image, suggest that the trigger introduces substantial changes as it does not maintain the overall statistical properties of the original image. The entropy $\text{H}$ is calculated using the histogram of pixel values across a set amount of images in a dataset:
$$H = -\sum_{i=1}^N p(i) \cdot \log_2 p(i),$$ 
where $p(i)$ is the probability of the $i$-th pixel value occurring in the dataset.

\begin{figure}[ht]
    \centering
    \includegraphics[width = 0.75\linewidth]{figures/NormalizedEntropy.png}
    \caption{Normalized entropy of the pixel values across all samples.}
    \label{fig:NormEntropy}
\end{figure}

\subsubsection{Number of activations per channel}
We explore the option of examining the average number of activations per channel in each frame of the images. The intuition behind this analysis is that including a large trigger in the image would significantly change the number of activations in the frames where it is present. 
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/activations1.png}
        \caption{Poison P=1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/activations1Mix.png}
        \caption{Mixed P=1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/activationsclean.png}
        \caption{Clean}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/activations3.png}
        \caption{Poison P=3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/activations3Mix.png}
        \caption{Mixed P=3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/activationsclean.png}
        \caption{Clean}
    \end{subfigure}
    
    \caption{Mean number of activations per channel and frame on poisoned, mixed, and clean samples where the trigger is inserted in the first frame with polarities 1 and 3.}
    \label{fig:meanAct}
\end{figure}

Additionally, we also examine the entropy of the average activation per frame. The concept is that frames containing triggers would exhibit similar activation numbers between them on the poisoned frames when compared to the clean frames.

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/entropy_activation_trig.png}
        \caption{Poisoned P=3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/entropy_activation_mix.png}
        \caption{Mixed P=3}
        
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/entropy_activation_base.png}
        \caption{Clean}
    \end{subfigure}
    \caption{Entropy of the number of activations in each frame of poisoned, mixed, and clean samples.}
    \label{fig:actEntropy}
\end{figure}

\subsubsection{Evaluation Results}
We evaluate these metrics in a test set consisting of 116 clean images and the same amount of poisoned ones. The poisoned samples are generated by inserting a full image trigger on the first frame with polarity $p=3$ of the clean set.

\begin{table}[ht]
    \caption{Evaluation of the stealthiness metrics on the clean and poisoned dataset.}
    \centering
    \begin{tabular}{ccc}
    \hline
    \multicolumn{2}{c}{\textbf{Metric}} & \textbf{Value} \\ \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{Mean Pixel Entropy}} & Clean & 0.87 \\
    \multicolumn{1}{c|}{} & Trigger & 0.81 \\
    Average MSE &  & 0.44 \\
    PSNR &  & 40.06 \\
    SSIM &  & 0.95 \\ \hline
    \end{tabular}
    
    \label{tab:stealth}
\end{table}

As seen in~\autoref{tab:stealth}, there is no obvious way to determine if the dataset contains poisoned samples. There is little difference in the pixel entropy between the clean and the poisoned samples (see~\autoref{fig:NormEntropy}). The average MSE could indeed be considered relatively high, but the PSNR, which is inversely related to the MSE, obtained a mark of 40.06; in this metric, anything above 40db is considered to be very good as it means that the reconstruction of the image contains little noise added. This difference in these two metrics is due to the nature of neuromorphic data, as its pixel values have no upper bound; each pixel contains the number of activations in a set amount of time. SSIM, on the other hand, obtained a value of 0.95, which indicates a nearly perfect structural similarity.

After seeing that these metrics were ineffective in discerning the poisoned samples, we focused on analyzing the number of activations per frame instead of the whole sample. Depending on the polarity and the size of the trigger, this could be a method of identifying a change in specific frames of some samples. However, when the polarity is set to $p=3$, which also obtained the best results on ASR in real-world environments (see~\autoref{tab:real-world}), it becomes much more challenging to discern the insertion of the triggers when the poisoned samples are mixed with the clean ones (see~\autoref{fig:meanAct}). It is also to be noted that this comparison was made using a ratio of 1:1 between clean and poisoned samples, when in reality, the dataset would contain only one poisoned sample for every ten clean ones, making it even harder to discern. 

When analyzing the entropy of each frame on a single sample by itself, we found that it is easy to discern the triggered frames when the size of the trigger represents the majority of the image, as the entropy of that frame would be very low or 0 if the trigger only contains a single value across the whole frame. However, this means that the user would need to analyze each frame of each sample by itself, which would be highly unpractical for large datasets or samples with more significant numbers of frames. If we apply this method to the whole dataset at once, we find no observable difference when comparing clean frames to the triggered ones (see~\autoref{fig:actEntropy}).

\todo{defense and stealthiness sections could be much shorter}
